Controlling diverse robots by inferring Jacobian fields with deep networks

Mirroring the complex structures and diverse functions of natural organisms is a long-standing challenge in robotics. Modern fabrication techniques have greatly expanded the feasible hardware, but using these systems requires control software to translate the desired motions into actuator commands. Conventional robots can easily be modeled as rigid links connected by joints, but it remains an open challenge to model and control biologically inspired robots that are often soft or made of several materials, lack sensing capabilities, and may change their material properties with use. Here, we introduce a method that uses deep neural networks to map a video stream of a robot to its visuomotor Jacobian field (the sensitivity of all 3D points to the robot's actuators). Our method enables the control of robots from only a single camera, makes no assumptions about the robots' materials, actuation, or sensing, and is trained without expert intervention by observing the execution of random commands. We demonstrate our method on a diverse set of robot manipulators that vary in actuation, materials, fabrication, and cost. Our approach achieves accurate closed-loop control and recovers the causal dynamic structure of each robot. Because it enables robot control using a generic camera as the only sensor, we anticipate that our work will broaden the design space of robotic systems and serve as a starting point for lowering the barrier to robotic automation.

==> tables/tabs_robot_cost/tab3_hsa_cost.tex <==
\begin{table}[]
\begin{tabular}{lcrr}
\hline
\multicolumn{1}{c}{\textbf{Part}}                                                                            & \textbf{Quantity} & \multicolumn{1}{c}{\textbf{Unit Cost}} & \multicolumn{1}{c}{\textbf{Total}} \\ \hline
ROBOTIS Dynamixel MX-28 servos                                                                               & 4                          & \$        259.00                       & \$    1,036.00                     \\
\begin{tabular}[c]{@{}l@{}}ROBOTIS Dynamixel starter kit\\ (USB hub, power board, power supply)\end{tabular} & 1                          & \$           59.70                     & \$           59.70                 \\
Carbon FPU 50 resin for pair of HSAs (114 ml)                                                                & 2                          & \$           28.43                     & \$           56.86                 \\
Carbon UMA 90 resin for adapters and end cap (168 ml)                                                        & 1                          & \$           25.15                     & \$           25.15                 \\
Acrylic sheet for servo casing (estimate)                                                                    &                            &                                        & \$              5.00               \\
Screws (estimate)                                                                                            &                            &                                        & \$              2.00               \\ \hline
\textbf{Grand Total}                                                                                         &                            &                                        & \textbf{\$        1,184.71}         
\end{tabular}
\caption{
Bill of materials for HSA platform.
}
% \vspace{-5pt}
\label{tab:table3_hsa_cost}
\end{table}

==> texts/introduction_old.tex <==
\section{Introduction}\label{sec1}

%%%%%%%%
Multi-material 3D printing has opened the door to the mass production of robots that do not require any human assembly. Compared to conventional robotic systems that cost tens to hundreds of thousands of dollars, 3D-printed, hybrid soft-rigid robots are extremely affordable at typically only hundreds of dollars, promising a future of widely accessible robotic automation for small businesses and organizations.

However, modeling and controlling hybrid soft-rigid robots is an unsolved problem. Conventional robots rely on sensors in every joint, jointed segment design with extreme rigidity, and high-precision manufacturing.
%
This reliance makes modeling and control simple for conventional robots. This, however, is exactly the reason for their exorbitant cost. 
%
On the other hand, state-of-the-art modeling approaches for hybrid soft-rigid robots involve an expert who designs a physical model of the robot. This expert-based process not only takes months or even years but is also hard to scale and non-transferable to other systems, as hybrid soft-rigid may change their physical properties due to long-term and irreversible effects, such as polymer degradation, crack formation, and weakening through cyclic loads \sz{cite}. 
%
To make affordable robotics a reality, we need new modeling and control algorithms that do not entirely rely on embedded sensors or hand-crafted physical models. 


%%%%
The difficulty of modeling a robotic system's kinematic and dynamic information arises from the deep coupling of a system's perception, geometry, and dynamics.
%
Traditional robots often bypass the modeling challenge by embedding a sparse set of angle sensors to infer the 3D kinematic and dynamic information.
%
This modeling strategy avoids directly perceiving and processing the dense, volumetric information about the state of the robotic system in the 3D world. 
%
Hence, for conventional robots, real-world customizations, such as mounting gripper cameras to a manipulation system and installing 3D-printed components, could make the 3D shape and inertial properties differ from the ideal configuration estimated at the time of manufacturing.
%
For hybrid soft-rigid systems, the conventional modeling strategy breaks down, as the system's 3D shape cannot be determined via a sparse set of sensors, and long-term irreversible physical effects exist, as mentioned above. Consequently, different sensing and modeling strategies have been individually proposed for each robotic system. For example, to sense a group of materials called handed shearing auxetics (HSA), past works have attempted to embed air channels, use a camera to record the interior, and fix a stretch sensor to the interior \lester{cite these works}.
%
In modeling, splines and piece-wise curvature have been employed to approximate the geometry of soft systems \lester{cite these works}.


%%%%%%%%
Another line of traditional solutions employs expensive motion capture systems, such as XXX, YYY \lester{cite motion capture system like OptiTrack, find RISP paper}. 
%
The cost of such motion capture systems often exceeds tens of thousands of dollars, making the solution inaccessible to low-resource robotics practitioners. 
%
This solution also relies on expert-guided decisions on where motion markers are placed \lester{cite some motion marker-based work}. 
%
As noted above, robotic platforms require dense and volumetric modeling of 3D geometry and dynamics. The sparse geometric information from motion capturing can be insufficient for robotic manipulation and motion planning applications.


%%%%%%%%
In contrast, humans have the ability to model and remote-control even the most imprecise of robots. 
%
Controlling the robot with just a video game controller, we can learn to pick and place objects within minutes, even with hybrid soft-rigid robots that are infeasible for conventional approaches to modeling and control.
%
Surprisingly, the only sensors we require are our eyes: From vision alone, humans reconstruct the robot’s 3D configuration, easily compensating for the lack of other sensor feedback and imprecision in motor movements. 
%
Within minutes of playtime, we infer a mental model that allows us to anticipate how the robot would move from any control input.


%%%%%%%%
Inspired by human perception, in this paper, we demonstrate a machine-learning model that is capable of controlling any robot from vision alone, without any prior assumptions of its 3D kinematics, dynamics, and sensorization.
%
Machine visual perception could capture rich kinematic and dynamic information about a robotic system. 
%
In particular, we rely on two major advancements in computer vision over the past decades in 3D reconstruction and motion representation.
%
First, progress in differentiable rendering has revolutionized 3D reconstruction. These techniques can characterize the geometry of a robotic system from just a collection of images, without any special-purpose imaging devices or prior knowledge of the shape of the system \s{Cite}.
%
Next, the dynamics of an unknown system require motion modeling that does not rely on expert knowledge. Recent methods from computer vision, such as optical flow and physical point tracking, promise dense motion estimation directly from videos \lester{Cite}.
%
Our model is trained on multi-view RGB-D video captured with several off-the-shelf cameras that observe the robot executing random actions. Subsequently, at test time, a single RGB image suffices to control the robot by defining the motion of any subset of 3D points, easily obtainable from a demonstration or manual input. In particular, our model enables control of robotic systems that were previously intractable, such as soft robots that can be 3D-printed for just hundreds of dollars and are both under-actuated and under-sensorized.

Our core contribution is a new 3D neural scene representation, the \textit{Jacobian Field}, that maps every 3D point to a representation of how that 3D point would move under any possible control input. 
%
The Jacobian Field extends the point-based Jacobian in traditional robotics that characterizes the motion of a sparse set of points, such as the tip of the end-effector, to a dense 3D field that characterizes the motion of \textit{every} 3D point. 
%
Our method is uniquely enabled by recent achievements in computer vision in neural scene representation, motion tracking, and differentiable rendering \lester{cite papers}. 
%

%%%%%%%%
In extensive real-world experiments, we demonstrate that our model enables control of diverse robotic systems, including a \$300 3D-printed hybrid soft-rigid pneumatic hand mounted on a UR5 arm \lester{cite}, soft actuators made from handed shearing auxetics \lester{cite}, and a 16 degrees-of-freedom Allegro hand \lester{cite}. 
%
Our experiments confirm that our model can be deployed for real-world applications and is robust against physical perturbation, visual occlusion, and background changes.
%
Our ablation study shows that our model is interpretable and learns the causal structure of the manipulator Jacobian that separates independent kinematic chains.
%
Our model opens the door towards a new generation of robotic systems that can forego conventional high-precision manufacturing and costly sensorization in favor of affordable, soft, under-actuated, and under-sensorized systems, dramatically lowering the barrier of entry to automation.
 

==> texts/outline.tex <==
\section{Outline}

\begin{itemize}
    \item Title: Include ``Neural Jacobian Field" in title?
\end{itemize}


\subsection{Abstract}

\begin{itemize}
    \item No more than 200 words
    \item See example: \url{https://www.nature.com/documents/nature-summary-paragraph.pdf}
\end{itemize}


\subsection{Main Text}

\begin{itemize}
    \item 2500 words, including abstract
    \item 4 figures
    \item No more than 50 references
    \item Subheadings up to 40 characters including spaces
\end{itemize}


\subsubsection{Introduction}
    
    123 text

\subsubsection{The Neural Jacobian Field}

\subsubsection{Results}
\begin{itemize}
    \item \textbf{Kinematics Prediction}

    123
    
    \item \textbf{Visuomotor Control}

    123
    
    \item \textbf{Robustness}

    Robustness to visual changes (occlusions, background changes), OOD scenarios (translations), external disturbances 
    
\end{itemize}

\subsubsection{Discussion}
Summarize results, discuss limitations, implications, impact


\subsection{Methods}

\begin{itemize}
    \item Typically not more than 3000 words, but more possible
\end{itemize}

\subsubsection{Robot Systems}
\begin{itemize}
    \item \textbf{Pneumatic Hand}

    3D printed in one piece, new, entirely soft, 5 DoF?, no sensors, pneumatically driven, costs \$300?

    Mounted on UR5, rigid, with 3 DoF?
    
    \item \textbf{Allegro Hand}

    off-the shelf, rigid with soft padding at fingertips, servo position feedback?, research and industry, 16 DoF? , costs \$15,000?
    
    \item \textbf{HSA Platform}

    3D printed HSAs, compliant, 4 DoF, mimics movements of human wrist plus elongation, servo-driven, servo position feedback but useless to predict state because compliant, material costs \$500? \todo{double check}
    
    \item \textbf{Poppy Ergo Jr}

    Ultra low-cost, DIY open-source platform (Poppy Project) for educational purposes, rigid, 6 DoF, assembled in 45 minutes, servomotor-driven, \textless\$300?
    
\end{itemize}

\subsubsection{Camera Setup}

\subsubsection{Data Collection}

\subsubsection{Neural Network Architecture and Training}

\subsubsection{Inference Procedure}

\subsubsection{Visuomotor Control}




\subsection{Supplementary Information}




==> texts/related.tex <==
\subsection{Related Work on Modeling and Control of Robots from Vision}
%
Yilun's paper on predicting optical flow and backing out actions with inverse kinematics.
%
Pieter's work on point tracking prediction.
%
Visual servoing for soft robots.
%
Hod Lipson's work.
%
Modeling continuous motion in cryo-EM. Recent methods for heterogeneous cryo-EM reconstruction have
explored the possibility of using linear [12, 44] and nonlinear [7, 11, 15, 29, 34, 36] mappings between
8 Levy et al.
latents and 3D structures. Nonlinear methods can be further categorized depending on the support they use
for representing density maps: neural networks [59, 60], 3D Zernike polynomials [19], Gaussian mixture
models [4, 61] or flow fields [45]. Normal mode-based approaches [16, 17, 23, 39] introduce a linear and
physically interpretable mapping between latents and atomic coordinates. However, these methods need a
coarse initialization of the density map or the poses to be provided by a pre-processing step of homogeneous
reconstruction. In practice, this ab initio step is error-prone due to (1) the presence of junk particles and (2)
large conformational motions or strong compositional heterogeneity. DRGN-AI runs directly on unposed
particle images and is therefore not subject to the above limitations.
